Shadow Unlearning: A Neuro-Semantic Approach to Fidelity-Preserving Faceless Forgetting in LLMs

Machine unlearning aims to selectively remove the influence of specific training samples to satisfy privacy regulations such as the GDPR's 'Right to be Forgotten'. However, many existing methods require access to the data being removed, exposing it to membership inference attacks and potential misuse of Personally Identifiable Information (PII). We address this critical challenge by proposing Shadow Unlearning, a novel paradigm of approximate unlearning, that performs machine unlearning on anonymized forget data without exposing PII. We further propose a novel privacy-preserving framework, Neuro-Semantic Projector Unlearning (NSPU) to achieve Shadow unlearning. To evaluate our method, we compile Multi-domain Fictitious Unlearning (MuFU) forget set across five diverse domains and introduce an evaluation stack to quantify the trade-off between knowledge retention and unlearning effectiveness. Experimental results on various LLMs show that NSPU achieves superior unlearning performance, preserves model utility, and enhances user privacy. Additionally, the proposed approach is at least 10x more computationally efficient than standard unlearning approaches. Our findings foster a new direction for privacy-aware machine unlearning that balances data protection and model fidelity.

==> table_compute_analysis.tex <==
% % % %Please add the following required packages to your document preamble:
% % % %\usepackage{graphicx}
% % \begin{table}[htb]
% % \centering\small
% % \label{tab:compute_analysis}
% % % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{lllll}
% % \toprule
% % Methods & LLaMA-7B & Mistral-7B & OLMoE-1B-7B & LLaMA-13B \\ \midrule
% % Retraining & 8.40 $\times$ $10^{22}$ & 3.36 $\times$ $10^{22}$  &  3.00 $\times$ $10^{22}$& 8.40 $\times$ $10^{26}$  \\
% % GA & 1.29 $\times$ $10^{17}$ & 1.29 $\times$ $10^{16}$   & 1.84$\times$ $10^{16}$ & 1.29 $\times$ $10^{21}$ \\
% % GD & 5.16 $\times$ $10^{17}$ & 5.16 $\times$ $10^{17}$  & 7.37 $\times$ $10^{16}$  & 5.16 $\times$ $10^{21}$  \\
% % KLM & 1.29 $\times$ $10^{17}$ & 1.29 $\times$ $10^{16}$  & 1.84$\times$ $10^{16}$  & 1.29 $\times$ $10^{21}$  \\
% % DPO & 5.16 $\times$ $10^{17}$ & 5.16 $\times$ $10^{17}$  & 7.37 $\times$ $10^{16}$  & 5.16 $\times$ $10^{21}$  \\
% % NPO & 5.16 $\times$ $10^{17}$ & 5.16 $\times$ $10^{17}$  & 7.37 $\times$ $10^{16}$  & 5.16 $\times$ $10^{21}$  \\
% % \rowcolor{lightgray}
% % \textbf{NSPU} &
% % $\boldsymbol{7.63 \times 10^{16}}$ &
% % $\boldsymbol{7.63 \times 10^{15}}$ &
% % $\boldsymbol{8.67 \times 10^{15}}$ &
% % $\boldsymbol{7.63 \times 10^{20}}$ \\ \bottomrule
% % \end{tabular}%
% % % }
% % \caption{Computational costs (FLOPs) across unlearning methods.}
% % \end{table}

% % %Please add the following required packages to your document preamble:
% % %\usepackage{graphicx}
% % \begin{table}[]
% % \centering\footnotesize
% % \label{tab:compute_analysis}
% % % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{lllll}
% % \toprule
% % Methods & LLaMA-7B & Mistral-7B & OLMoE-1B-7B & LLaMA-13B \\ \midrule
% % Retraining & 8.40 $\times$ $10^{22}$ & 3.36 $\times$ $10^{22}$  &  3.00 $\times$ $10^{22}$& 8.40 $\times$ $10^{26}$  \\
% % GA & 1.29 $\times$ $10^{17}$ & 1.29 $\times$ $10^{16}$   & 1.84$\times$ $10^{16}$ & 1.29 $\times$ $10^{21}$ \\
% % GD & 5.16 $\times$ $10^{17}$ & 5.16 $\times$ $10^{17}$  & 7.37 $\times$ $10^{16}$  & 5.16 $\times$ $10^{21}$  \\
% % KLM & 1.29 $\times$ $10^{17}$ & 1.29 $\times$ $10^{16}$  & 1.84$\times$ $10^{16}$  & 1.29 $\times$ $10^{21}$  \\
% % DPO & 5.16 $\times$ $10^{17}$ & 5.16 $\times$ $10^{17}$  & 7.37 $\times$ $10^{16}$  & 5.16 $\times$ $10^{21}$  \\
% % NPO & 5.16 $\times$ $10^{17}$ & 5.16 $\times$ $10^{17}$  & 7.37 $\times$ $10^{16}$  & 5.16 $\times$ $10^{21}$  \\
% % \rowcolor{lightgray}
% % \textbf{NSPU} &
% % $\boldsymbol{7.63 \times 10^{16}}$ &
% % $\boldsymbol{7.63 \times 10^{15}}$ &
% % $\boldsymbol{8.67 \times 10^{15}}$ &
% % $\boldsymbol{7.63 \times 10^{20}}$ \\ \bottomrule
% % \end{tabular}%
% % % }
% % \caption{Computational costs (FLOPs) across unlearning methods.}
% % \end{table}

% \begin{table}[]
% \centering\footnotesize
% \label{tab:compute_analysis}
% \setlength{\tabcolsep}{2pt}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lllll}
% \toprule
% Methods & LLaMA-7B & Mistral-7B & OLMoE-7B & LLaMA-13B \\ \midrule
% Retraining & 8.4 $\times$ $10^{22}$ & 3.4 $\times$ $10^{22}$  &  3.0 $\times$ $10^{22}$& 8.4 $\times$ $10^{26}$  \\
% GA & 1.3 $\times$ $10^{17}$ & 1.3 $\times$ $10^{16}$   & 1.8$\times$ $10^{16}$ & 1.3 $\times$ $10^{21}$ \\
% GD & 5.2 $\times$ $10^{17}$ & 5.2 $\times$ $10^{17}$  & 7.4 $\times$ $10^{16}$  & 5.2 $\times$ $10^{21}$  \\
% KLM & 1.3 $\times$ $10^{17}$ & 1.3 $\times$ $10^{16}$  & 1.8$\times$ $10^{16}$  & 1.3 $\times$ $10^{21}$  \\
% DPO & 5.2 $\times$ $10^{17}$ & 5.2 $\times$ $10^{17}$  & 7.4 $\times$ $10^{16}$  & 5.2 $\times$ $10^{21}$  \\
% NPO & 5.2 $\times$ $10^{17}$ & 5.2 $\times$ $10^{17}$  & 7.4 $\times$ $10^{16}$  & 5.2 $\times$ $10^{21}$  \\
% \rowcolor{lightgray}
% \textbf{NSPU} &
% $\boldsymbol{7.6 \times 10^{16}}$ &
% $\boldsymbol{7.6 \times 10^{15}}$ &
% $\boldsymbol{8.7 \times 10^{15}}$ &
% $\boldsymbol{7.6 \times 10^{20}}$ \\ \bottomrule
% \end{tabular}%
% % }
% \caption{Computational costs (FLOPs) across unlearning methods.}
% \end{table}










